Online Graph Completion: Multivariate Signal Recovery in Computer Vision

The adoption of "human-in-the-loop" paradigms in computer vision and machine learning is leading to various applications where the actual data acquisition (e.g., human supervision) and the underlying inference algorithms are closely interwined. While classical work in active learning provides effective solutions when the learning module involves classification and regression tasks, many practical issues such as partially observed measurements, financial constraints and even additional distributional or structural aspects of the data typically fall outside the scope of this treatment. For instance, with sequential acquisition of partial measurements of data that manifest as a matrix (or tensor), novel strategies for completion (or collaborative filtering) of the remaining entries have only been studied recently. Motivated by vision problems where we seek to annotate a large dataset of images via a crowdsourced platform or alternatively, complement results from a state-of-the-art object detector using human feedback, we study the "completion" problem defined on graphs, where requests for additional measurements must be made sequentially. We design the optimization model in the Fourier domain of the graph describing how ideas based on adaptive submodularity provide algorithms that work well in practice. On a large set of images collected from Imgur, we see promising results on images that are otherwise difficult to categorize. We also show applications to an experimental design problem in neuroimaging.

==> intro.tex <==
\section{Introduction}
%intro...

The problem of missing data is ubiquitous in data science. 
In typical scientific studies, 
data are first collected for various ambitious purposes. 
However in practice, there are many obstacles in the data acquisition process (e.g., budget constraint, equipment malfunction, human introduced error and noise) 
which yield either missing or meaningless measurements.   
%therefore many datasets end up with missing measurements. 
This becomes a serious problem in the experimental design phase, 
where many of the samples with partially missing data are often discarded or synthetic data are imputed to fill in the blanks \cite{efron1994missing,rubin1976inference}. 
When these missing data are not carefully handled especially without knowing the source of the missingness, 
its downstream analyses will introduce bias or strongly affect its statistical outcome \cite{allison2001missing}. 
In any case, without the ability to fully utilize the data, 
the follow-up analysis eventually ends up with sub-optimal results with significantly decreased statistical power. 
%not being able to full utilization of the data
%% In many cases, Even after collecting for ambitious objectives, 
%% a substantial 
%% Depending on how the data are missing (e.g., missing at random and missing based on unobserved predictor), traditional approaches impute the missing data or perform regression to fill in the missing data. 

To deal with the issues of missing data, matrix completion methods are broadly deployed in computer vision and machine learning.
%to deal with the issues of missing data. 
Based on a few theoretical assumptions such as restricted isometry property (RIP) and incoherent sampling, 
the de facto ways of matrix completion have led to resurgence in analysis of factorization forms \cite{candes2009exact,yu2009fast,candes2009exact,cai2010singular}, 
which on its own has a long history since early 1990s \cite{tomasi1992shape}. 

Now, consider a variation of this problem where the structure is slightly harder to capture in terms of parsimony. 
That is, a matrix (or an image) has a nice regular structure to begin with, 
but the question is whether we can work on a similar task without the regularity in the domain. 
Such a complex domain is generally represented 
as a graph with vertices representing data points and edges that are connecting them, 
and measurements are defined as signals on the vertices. 
When $N$ number of graph vertices are enumerated and corresponding multi-variate measurements of size $p$ are laid next to each other, 
they compile a form of matrix of size $N \times p$. 
With missing measurements in this matrix, it clearly yields a matrix completion problem. 
However in this case, the data are missing at certain rows instead of random locations and the relationships between elements no longer hold as in traditional matrix completion. 
In this regime, the aforementioned assumptions become ambiguous and it becomes difficult to achieve a feasible solution for 
this {\em graph completion problem}. 

\begin{figure}[!tb]
  \centering
  \includegraphics[width = .12\textwidth]{fig/arma_mesh}
  \includegraphics[width = .235\textwidth]{fig/arma_samples}
  \includegraphics[width = .235\textwidth]{fig/arma_f}
  \caption{\footnotesize An example of graph completion. Given a graph and partial measurements on the vertices (left), reconstruct the whole signal (right). }
\end{figure}

These issues were recognized in recent works where collaborative filtering was generalized to graphs \cite{rao2015collaborative}  
and random sampling scheme with bandlimit assumption was introduced \cite{puy2015random}.  
These methods essentially approach the problem using diffusion process %which is a smoothing operation 
by propagating observed measurements to their neighboring vertices where the measurements are unobserved. 
%% A similar operation was also acknowleged for semi-supervised learning problem on graphs as well, 
%% where known labels are propagated to the vertices with unknown labels \cite{kim}. 
%In either approaches, 
They utilize the spectrum of the Laplacian of a graph to simulate the diffusion process 
in the native space (i.e., a graph), 
and solve an optimization problem in the graph space to achieve the optimal solution. 
%We would like to explore the same 
Although these methods have paved the way to generalize 
traditional signal recovery problems to a graph domain, 
these solvers do not take advantage of the bandlimited nature of signals nor the low-rank property 
as in other matrix completion approaches.  

As soon as we look at many of the problems in computer vision, 
we find that this type of problems are addressed more than before. 
Advances in object detection algorithms are yielding high accuracy in single images yet  
having difficulties in cases with severe occlusion or ambiguity. 
Recent literature suggest that such failure cases may be helped by accessing the relationships between the images 
through metadata (e.g., text, image features and social interactions) where images are represented as vertices and the relationships establish connections between the images \cite{yang2016improving,kim2016semi}. 
%(e.g., image features, text features from captions/comments). 
In addition, imagine the same situation as above but ``measurement task'' would be more complicated by ``the man in the loop''. 
For example, the dataset for Visual Question Answering (VQA) contains open-end 760000 questions and 10 million answers 
which were collected by human intervention via Amazon Mechanical Turk. 
There is a significant financial aspect here when we have to offer costly ``supervision'' for each measurement, 
and one would obviously want to maximize the ``return'' on the investment.  
%% we would have to design the best policy as possible 
%% within our budget constraint. 
If one could cut down the number of data acquisition process by half and is still able to 
answer what the measurement would be on the other unobserved half, 
there is a substantial benefit in terms of both cost and statistical power. 
Such a benefit can be even more emphasized for neuroimaging studies 
where we have to recruit a number of participants to acquire costly (imaging or non-imaging) data 
but typically end up with many missing elements with human error and complicated preprocessing steps. 

% how we approach this problem...
Apart from this setting, the reader will see that given the pervasiveness of experimental design in computer vision, 
such a model is broadly applicable. 
For an effective and efficient way to approach this problem, 
we also look at the harmonic analysis of the graph 
but we utilize the parsimonious representations in Fourier/wavelet space for graphs. 
In general, measurements/signals are represented as a smooth function in their native space 
but their representation in a dual space (e.g., frequency space) may be sparse: 
this has been the foundation of intuition for Fourier/wavelet analysis in signal processing and sparse coding/matrix completion in machine learning and computer vision.  
In addition, what is even more interesting is the ``online'' version of this problem. 
As soon as we acquire one measurement, the utility function is adjusted and will update the remainder to affect our ``policy'' to acquire the next measurement.  
While related to the idea of diminishing returns, this is an adaptive variation, which poses interesting technical challenges
in terms of optimization and active learning. 
Such an online scenario has been studied for a general matrix or tensor setting \cite{krishnamurthy2013low,kumar2012sampling} but not on a graph. 
We will show how recent work can be adopted for analysis of measurements on a graph in an online manner 
utilizing the Fourier space of the graph. 

The contribution of this paper is to provide a framework for choosing the optimal policy of selecting vertices in a graph 
in an active learning setting (i.e., online manner) which will benefit recovery of unobserved measurements using harmonic analysis for graphs. 
%sharmonic analysis inspired algorithm to estimate band-limited signals that are defined on graphs.
%It turns out that such solutions %, when available,
%directly yield an efficient procedure to conduct adaptive queries for designing experiments involving stratified costs of measurements,
%i.e., where the first subset of measures is free whereas the second set of $(p- p^\prime)$ measures
%is expensive and must be requested for a small fraction of participants.
Our framework use a recent theory on adaptive submodularity for the selection of policy using a greedy algorithm, 
and provide an efficient solver to recover measurements on graphs by exploring its natural properties in an analogue of Fourier space for graphs. 
%relies on the design of an efficient decoder to recover the band-limited
%original signal involving multiple channels which was only partially observed.
%which will facilitate statistical analysis of neuroimages that are facing problems due to small sample size.
%Such a framework is
In order to accomplish these goals, the paper makes the following contributions.
\begin{compactenum}[\bfseries (i)]
\item We propose an algorithm to decide the optimal policy using adaptive submodularity on graphs.
\item We show how a multi-variate measurements on a graph can be estimated by exploring its sparse representation in its dual space. %with only a few observations via a simple optimization scheme.
\item We provide an extensive set of experiments on {\em three independent datasets} to evaluate our framework for computer vision problems by
  solving active learning problems to estimate multiple object labels in images based on their relationships as well as 
  for a neuroimaging problem where we perform regression on multi-variate measurements in different brain regions. 
\end{compactenum}


%% \begin{itemize}
%% \item The problem of missing data is ubiquitous in science. 
%% \item Traditional approaches...
%% \item Matrix completion is broadly deployed in computer vision and machine learning in the last decade.
%% \item De facto ways has lead to resurgence in analysis of factorization forms, which on its own has a long history in vision since Tomasi-Kanade. 
%% \item These approaches are adopted for problems that do not deal with missing data. 
%% \end{itemize}

%% \begin{itemize}
%% \item Consider a variation of this problem where the structure is slightly harder to capture in terms of parsimony which is not obvious. 
%% \item Completion problem on graphs solved by diffusion process (smoothing operation). 
%% \item Or we can try to utilize/explore analysis of matrix completion on this type of structure. 
%% \end{itemize}

%% \begin{itemize}
%% \item Why should we care?
%% \item Ex 1) Images, object detectors, similarity between nodes based on comments where object detectors fail, we still want to succeed. 
%% \item Ex 2) Imagine the same situation as before, but ``measurement task'' would be something more complicated by ``the man in the loop''. Visual Question Answering...
%% There is a financial aspect to this. Assume we offer money to ``supervision'' how can we maximize ``return'' on investment. 
%% \item Ex 3) Neuroimaging aspect...
%% \end{itemize}

%% \begin{itemize}
%% \item Apart from this setting, the reader will see that given the pervasiveness of experimental design in computer vision: the model is very broadly applicable. 
%% \item We look at the harmonic analysis of the graph... parsimony in Fourier/wavelet space. 
%% \item But what is more interesting is that ``online'' version of this problem. 
%% \item As soon as we acquire one measurement, the utility function changes and will inform the remainder of our ``policy''. 
%% \item While related to the idea of diminishing returns, this is an adaptive variation, which poses interesting technical challenges. 
%% \item We show how recent work can be adopted for analysis of signals in the Fourier space of graphs. 
%% \end{itemize}

%% Contributions...
%% \begin{itemize}
%% \item Technical aspect: online graph, adaptive submodularity
%% \item Experiments: MS-coco / Imgur dataset is interesting by itself
%% \item Neuroimaging experiment: as in eccv 
%% \end{itemize}

